HAIChart: Human and AI Paired Visualization System

The growing importance of data visualization in business intelligence and data science emphasizes the need for tools that can efficiently generate meaningful visualizations from large datasets. Existing tools fall into two main categories: human-powered tools (e.g., Tableau and PowerBI), which require intensive expert involvement, and AI-powered automated tools (e.g., Draco and Table2Charts), which often fall short of guessing specific user needs. In this paper, we aim to achieve the best of both worlds. Our key idea is to initially auto-generate a set of high-quality visualizations to minimize manual effort, then refine this process iteratively with user feedback to more closely align with their needs. To this end, we present HAIChart, a reinforcement learning-based framework designed to iteratively recommend good visualizations for a given dataset by incorporating user feedback. Specifically, we propose a Monte Carlo Graph Search-based visualization generation algorithm paired with a composite reward function to efficiently explore the visualization space and automatically generate good visualizations. We devise a visualization hints mechanism to actively incorporate user feedback, thus progressively refining the visualization generation module. We further prove that the top-k visualization hints selection problem is NP-hard and design an efficient algorithm. We conduct both quantitative evaluations and user studies, showing that HAIChart significantly outperforms state-of-the-art human-powered tools (21% better at Recall and 1.8 times faster) and AI-powered automatic tools (25.1% and 14.9% better in terms of Hit@3 and R10@30, respectively).

==> src/demo.tex <==
%!TEX root = ../main.tex
%\vspace*{-1em}
\subsection{System Demonstration}
\label{sec:demo}

% We provide users with a web interface designed to facilitate visualization exploration more conveniently. In this web interface, we primarily demonstrate two scenarios: (1) First-Round Visualization Recommendations, and (2) Multi-Round Visualization Recommendation based on Hints.

We implemented the \sys, a web-based interface designed to facilitate visualization exploration, as shown in Figure~\ref{fig:screenshot}. In this interface, we demonstrate two main scenarios: (1) First-Round Visualization Recommendations, and (2) Multi-Round Visualization Recommendations based on Hints.


\stitle{Datasets.} We utilize the \textit{Flight Delay Statistics} dataset, which comprises records including the date, carrier, destination city (\textit{destcity}), departure delay (\textit{depdelay}), arrival delay (\textit{arrdelay}), and the number of passengers. This dataset allows us to analyze various factors contributing to flight delays.

% Next, we'll illustrate the key features of \sys by analyzing the \textit{Flight Delay Statistics} dataset. 

\stitle{First-Round Visualization Recommendations.} Initially, users upload their dataset. \sys then displays the data fields of the table, allowing users to explore further by clicking on fields of interest. \sys also logs users' historical actions, making it easier to retrieve previous analyses, as shown in Figure~\ref{fig:screenshot}-~\ding{182}.

After uploading the dataset, \sys employs a Monte Carlo Graph Search algorithm guided by a composite reward function to automatically recommend a series of high-quality visualizations. As illustrated in Figure~\ref{fig:screenshot}-~\ding{183}, the initial recommendations include a scatter plot revealing the relationship between flight arrival delays (\textit{arrdelay}) and departure delays (\textit{depdelay}), and a bar plot showing the relationship between carriers and passengers. These visualizations help users quickly grasp key information within the dataset, providing an intuitive analytical perspective on various factors contributing to flight delays.

To enhance the user experience, \sys supports interactive operations on visualizations, such as zooming, switching chart types, and viewing underlying data (Figure~\ref{fig:screenshot}-~\ding{183}). These features enrich the visualization editing experience and enable thorough exploration and analysis of the data, uncovering potential insights.

\stitle{Multi-Round Visualization Recommendations based on Hints.}
Existing interactive visualization tools, such as Voyager2~\cite{wongsuphasawat2017voyager}, require users to iteratively refine visualizations through complex control panels. In contrast, \sys simplifies data exploration with visualization hints. This feature recommends hints, enabling users to bypass cumbersome decisions and explore data via a multiple-choice format, lowering barriers to data exploration.

For instance, users can explore analysis directions by browsing hints recommended by \sys after viewing initial visualizations. As shown in Figure~\ref{fig:screenshot}-~\ding{184}, users interested in “{\sf Compare {\tt arrdelay} to different categories}” can select this hint. \sys then optimizes recommendations based on “{\tt arrdelay}” and records user preferences, as demonstrated in Figure~\ref{fig:screenshot}-~\ding{185}. Using the Monte Carlo Graph Search algorithm and constrained search techniques, \sys provides high-quality visualizations related to “{\tt arrdelay},” such as a stacked bar chart comparing “{\tt arrdelay}” across different destination cities and a line chart showing “{\tt arrdelay}” trends over time (Figure~\ref{fig:screenshot}-~\ding{186}). \sys continuously refines recommendations based on user preferences and data features, offering an intuitive interface for data exploration.


% For example, after viewing the initial recommended visualizations, users can explore interesting analysis directions by browsing through visualization hints recommended by \sys. As shown in Figure~\ref{fig:screenshot}-~\ding{184}, if users are interested in ``{\sf Compare {\tt arrdelay} to different categories},'' they can select this hint. \sys then optimizes the recommendation strategy based on the selected “{\tt arrdelay}” and records user preferences, as demonstrated in Figure~\ref{fig:screenshot}-~\ding{185}. By leveraging the Monte Carlo Graph Search algorithm combined with constrained search techniques, \sys provides high-quality visualizations related to ``{\tt arrdelay}''. Examples include a stacked bar chart comparing ``{\tt arrdelay}'' across different destination cities and a line chart showing trends of ``{\tt arrdelay}'' over time, as shown in Figure~\ref{fig:screenshot}-~\ding{186}. Additionally, \sys continuously refines its recommendations based on the user's current preferences and data features, further simplifying the data exploration process and offering an intuitive and easy-to-use interface for data exploration.



==> src/revision.tex <==
%!TEX root = ../main.tex
\subsection*{Dear VLDB Meta-Reviewer and Reviewers:} 

%\etitle{1:} Do a comparison with PI2
%
%
%\etitle{2:} Improve the discussion of the design:
%\begin{itemize}
%	\item Improve the analysis of MCGS to MCTS
%	\item Explain why a GAN is necessary
%	\item Justify the problem definition
%\end{itemize}
%\etitle{3:} Improve the experiments to
%\begin{itemize}
%	\item Explain what training data is used
%	\item Complete a sensitivity analysis of the parameters
%	\item Cover more of the framework
%	\item Use more diverse datasets
%\end{itemize}
%\etitle{4:} Improve the user study to
%\begin{itemize}
%	\item Better compare to state of the art approaches
%	\item Model user involvement and effort
%	\item Include qualitative analysis
%	\item Either motivate why only experts were included or expand the study to include non-experts
%\end{itemize}

Thank you for the encouraging comments and suggestions. The paper has been significantly improved based on the constructive feedback. The revised parts in the paper are highlighted in \add{blue}. 

First, we have added the following new experiments in \textbf{Sec~\ref{sec:experiment}}.

\begin{enumerate}
    \item[(\textbf{E1})] \textit{Ablation Study of the MCGS Optimization Techniques.} To evaluate the MCGS optimization techniques, including \textit{rule-based pruning} and the \textit{adaptive random exploration strategy}, we conducted an ablation study. The results show that \textit{rule-based pruning} improves recommendation quality by ensuring visualizations are syntactically correct. Meanwhile, the \textit{adaptive random exploration strategy} enhances diversity and prevents local optima by introducing random noise. This strategy serves as a complement to UCB, thereby improving recommendation performance (\textbf{Exp-4}, Table~\ref{tab:ablation_study}).
    \item[(\textbf{E2})] \textit{Parameter Sensitivity Analysis for MCGS.} We evaluated the impact of the UCB balance parameter \(c\) and the number of iterations \(n\). Results show the algorithm is stable and performs well across different settings, demonstrating parameter insensitivity within a certain range (\textbf{Exp-6}, Figure~\ref{fig:parameter_results}).
    \item[(\textbf{E3})] \textit{Parameter sensitivity analysis for Visualization Hints Selection.} We conducted a sensitivity analysis for Visualization Hints Selection, focusing on \( k \) (number of hints), \( B \) (budget), and \( l \) (number of visualizations per hint). The experiment shows that optimal settings for these parameters can enhance the quality of recommendations while balancing cost and effectiveness (\textbf{Exp-6}, Figure~\ref{fig:hints_selection_parameter_analysis}).
    \item[(\textbf{E4})] \textit{User Study Enhancements.} We have extended our user study to include non-experts, demonstrating that \sys is suitable for both expert and non-expert users. Additionally, we refined the LLM4Vis~\cite{DBLP:conf/emnlp/WangZWLW23} by improving its prompt, enabling better data queries and top-$k$ visualization recommendations. We named this improved tool LLM4Vis+. In the user study, we compared \sys with LLM4Vis+ and found that \sys, with its automatic visualization recommendations and corresponding hints, is more efficient and lowers the barrier for users compared to the natural language interaction required by LLM4Vis+ (\textbf{Exp-2}, Table~\ref{tab:multi-turn_results}, Figure~\ref{fig:user_study}, Figure~\ref{fig:user_inter}).
    % \item[(\textbf{E4})] \textit{User Study Enhancements.} We have extended our user study to include non-experts, demonstrating that \sys is suitable for both expert and non-expert users (\textbf{Exp-2}).
    \item[(\textbf{E5})] \textit{Efficiency Comparison of MCGS and MCTS.} We compared the efficiency of MCGS and MCTS, \ie~ \sys using MCGS and MCTS, respectively. The results show that \sys (using MCGS), on average, is 1.8 times faster than \sys (using MCTS), particularly for datasets with many columns. For example, when processing the VideoGame dataset with 15 columns, \sys's graph-based structure is 2.9 times faster than MCTS's tree-based structure  (\textbf{Exp-7}, Figure~\ref{fig:efficiency_results}).
    \item[(\textbf{E6})] \textit{Training \sys using VizML.} To ensure fair comparison, we trained the data features of the reward function using VizML, naming this version \sys-. Comparisons with state-of-the-art methods demonstrated that \sys- outperformed them overall (\textbf{Exp-1}, Table~\ref{tab:init_rec_results}).
\end{enumerate}

Second, we have also made the following main changes:

\begin{enumerate}
    \item[(\textbf{C1})] We conducted a detailed comparison of the MCTS and MCGS methods, demonstrating the effectiveness of MCGS as detailed in \textbf{Sec~\ref{sec:mcgs_vis_gen}}.
    \item[(\textbf{C2})] {We further clarified the reasons for introducing optimization techniques in MCGS, including \textit{rule-based pruning} and \textit{adaptive random exploration strategy}, as detailed in \textbf{Sec~\ref{sec:optim}}.}
    \item[(\textbf{C3})] We have added detailed explanations about the choice of GANs and their implementation methods, found in \textbf{Sec~\ref{sec:learn_reward_function}}.
    \item[(\textbf{C4})] We included new statistical information about the VizML dataset in \textbf{Sec~\ref{sec:exp_settings}}. This demonstrates that VizML is the largest benchmark dataset in the visualization field, encompassing a large-scale, cross-domain collection of real user data and their created visualizations.
    \item[(\textbf{C5})] In \textbf{Sec~\ref{sec:exp_multi_round}}, we provided additional details on the user study, including the number of hints, types of feedback, and the scope of \sys usage. We also conducted a qualitative analysis of user comments.
    \item[(\textbf{C6})] In \textbf{Sec~\ref{sec:related}}, we enhanced the discussion of related work, particularly focusing on comparisons with PI2.   
\end{enumerate}

\subsection*{Responses to Meta-Reviewer} 

Based on the above new experiments ({\bf E1--E6}) and major changes ({\bf C1--C6}), we have addressed all revision changes required by the meta-reviewer, including: 

\be
    \item Do a comparison with PI2;
    \item Improve the discussion of the design; and
    \item Improve the experiments and user study.
\ee

Please see our detailed responses to all the reviewers below.


\subsection*{Responses to Reviewer \#3} 

\etitle{WEAK POINT W1:} \textit{Certain elements of the framework are not covered in the experiments, making their impact on the overall framework somewhat unclear. }

\etitle{DETAIL D1:} \textit{The framework incorporates numerous elements, such as the use of MCGS and UCB for search, rule-based pruning of visualizations, random exploration, and incorporating user feedback in the form of hints. While some are evaluated in the experiments, the tuning of certain elements (e.g., exploration vs. exploitation) or the role of others (e.g., rule-based pruning and random exploration) is not fully explored in the study. Additional experiments or a more intuitive explanation of these components could enhance understanding of their roles within the entire framework. {For example, the necessity of random exploration when UCB already includes exploration parameters}, or {the effectiveness of strategies for addressing the cold start problem, is a bit unclear}.}

\res{Thank you for the constructive feedback. 
	We have conducted new experiments (\textbf{Exp-4}, \textbf{Exp-5}, and \textbf{Exp-6} in \textbf{Sec~\ref{sec:experiment}}) to explore the impact of each component on the \sys.

Specifically, we have included ablation studies (\textbf{Exp-4 and Exp-5}) to explore the effects of \textit{rule-based pruning}, \textit{random exploration}, and \textit{the user preferences model}.
%
The key findings are as follows:

\stab (1) Rule-based pruning ensures the validity of the generated visualizations, \ie generating syntactically correct visualizations.

\stab (2) Our adaptive random exploration avoids local optima by introducing new random noise (\ie exploring diversified visualization results), complementing existing exploration parameters in UCB.

\stab (3) The user preferences model alleviates cold start problems in visualization recommendation scenarios by learning general user preferences based on the GAN model.

We have clarified these parts in \textbf{Sec~\ref{sec:rl}} and \textbf{Sec~\ref{sec:reward}}.

In addition, we have conducted new experiments (\textbf{Exp-6}) to analyze the tuning of certain elements of \sys. 
Specifically, for the trade-off between exploration and exploitation, \sys works effectively when the balance factor \(c\) in UCB within the range \([0.5, 2.5]\), achieving the best results with a setting of \(1.5\).
}


\etitle{WEAK POINT W2:} \textit{The experiments use two datasets with specific characteristics. To ensure the generalizability of the results, more diverse datasets are needed. }

\etitle{DETAIL D2:} \textit{Two datasets, VizML and KaggleBench, with specific characteristics are used. VizML, for instance, appears to have very simple datasets, with only 2 charts per dataset and 3-4 columns per table. It's uncertain whether these datasets possess the complexity of visualization search that the authors aim to address. Including more diverse datasets could give stronger evidence to the significance of the results.}

\res{Thanks for the comment and sorry for the confusion. The VizML corpus, a large-scale and cross-domain visualization dataset for visualization recommendation tasks, is widely used by previous works such as PVisRec~\cite{qian2022personalized}, Table2Charts~\cite{zhou2021table2charts}, KG4VIS~\cite{li2021kg4vis}, and LLM4Vis~\cite{DBLP:conf/emnlp/WangZWLW23}.
VizML contains \textbf{79,475 tables} and \textbf{162,905 visualizations} from the real-world scenarios. On average, each table contains two visualizations \textit{created by real users}, with a maximum of 144 visualizations and up to 25 columns. This diversity and extensive coverage across various domains support our results comprehensively. For more detailed statistics, please refer to Table~\ref{tab:experimental_datasets}, Table~\ref{tab:multi-turn_datasets}, and Figure~\ref{fig:vizml_statistical} in \textbf{Sec}~\ref{sec:exp_settings}.
}
	
%The VizML corpus, widely used in visualization recommendation evaluations such as PVisRec~\cite{qian2022personalized}, Table2Charts~\cite{zhou2021table2charts}, KG4VIS~\cite{li2021kg4vis}, and LLM4Vis~\cite{DBLP:conf/emnlp/WangZWLW23}, is known for its large scale, cross-domain, and diverse characteristics. It is currently the largest benchmark in the visualization field, containing 79,475 tables and 162,905 visualizations from the real-world scenarios. On average, each table contains two visualizations, with a maximum of 144 visualizations and up to 25 columns. This diversity and extensive coverage across various domains support our results comprehensively. For more detailed statistics, please refer to Tables~\ref{tab:experimental_datasets}, Tables~\ref{tab:multi-turn_datasets}, and Figure~\ref{fig:vizml_statistical} (\textbf{Sec~\ref{sec:experiment}}).}
% We have now added statistical information for the VizML and KaggleBench corpora, which are both diverse and extensive across various domains. These datasets are comprehensive and support our results. For more detailed statistics, please refer to Tables~\ref{tab:experimental_datasets}, Tables~\ref{tab:multi-turn_datasets}, and Figure~\ref{fig:vizml_statistical} (\textbf{Sec~\ref{sec:experiment}}).


\etitle{WEAK POINT W3:} \textit{A crucial component is user involvement and effort, which is not adequately modeled in the experiments to measure value for money and the performance gain for user effort.}

\etitle{DETAIL D3:} \textit{A significant aspect of the framework is the integration of user feedback with automatic recommendation methods, distinguishing this work from existing research. The study examines user input in the form of hints, yet the experiments mainly focus on rounds of interaction. It's unclear how many hints are received in each round (is it the number ``k'' in hint selection, and what is the specific value in the experiments?). Including more detail on the user effort required within the framework could clarify the value derived from user involvement.}

\res{Sorry for the confusion. Indeed,  the $k$ refers to the total number of hints in each round, and we specified  $k$ as 9 in the user study.

Additionally, we conducted new experiments (\textbf{Exp-6}) to examine how different values of $k$ affect overall performance, as suggested.
As shown in Figure~\ref{fig:hints_selection_parameter_analysis}(b),   a lower $k$ (\eg $k$=3) fails to capture users' interests effectively, while a larger $k$ (\eg $k$=15) leads to higher user effort with limited improvement in benefit. Therefore, setting $k$ to 9 strikes a better balance between benefit and user effort.
}



\subsection*{Responses to Reviewer \#4} 

\etitle{WEAK POINT W1:} \textit{The paper did not discuss PI2 which explores an even harder problem of interactive UI generation and employs Monte Carlo Tree Search-based method for generation and incorporates user feedback via query refinement. While goal of both work is slightly different, the motivation is somewhat similar. The related work discussion should clarify the similarities and differences between the two work.}

\res{Thank you for the suggestion. We have discussed the connections between PI2~\cite{DBLP:conf/sigmod/Chen022} and our system in the related work section (\textbf{Sec}~\ref{sec:related}).
Generally speaking, PI2 is a system based on MCTS that generates an interactive UI from a set of SQL logs, helping developers understand the queries needed for a desired analysis task. PI2 requires users to provide the SQL queries needed for analysis tasks, while \sys automatically recommends visualizations based on the user’s dataset. In terms of interaction, PI2 allows users to refine query results through UI widgets, whereas \sys introduces visualization hints to guide users in data exploration. {\em While both systems aim to facilitate data exploration, their application scenarios differ.}}


\etitle{WEAK POINT W2:} \textit{The user study design lacks sufficient details. The ``Procedure'' paragraph mentions collecting user feedback and comments. However, what type of feedback was collected and how were they determined. The paper also missing any qualitative analysis of user comments --- such comments are often crucial in understanding user experience and characterizing the strengths and weaknesses of the system. Such details should be included in evaluation.}

\res{
Thanks for the good suggestion. We have revised the ``Procedure'' part to detail the types and selection criteria of user feedback collected, and included a qualitative analysis of user comments to describe the strengths and weaknesses of \sys.
	
%In the revised manuscript, we now specify that the feedback collected includes both structured and unstructured types. Structured feedback was gathered through a predefined questionnaire assessing various aspects such as usability, efficiency, and overall satisfaction. Unstructured feedback was collected through open-ended questions and free-form comments, allowing participants to express their thoughts and suggestions in their own words.

The qualitative analysis of user comments indicates that participants widely acknowledged that \sys, by providing hints that guide further exploration, not only simplifies the data exploration process but also enhances analysis efficiency. However, they also pointed out limitations, such as the need for a control panel for custom field selection to increase its flexibility.

For more details, please see the updated ``Procedure'' paragraph and the qualitative analysis in \textbf{Exp-2}. We believe these additions provide a more comprehensive understanding of user experiences and the strengths and weaknesses of our system.}

\etitle{WEAK POINT W3:} \textit{The scope of ~\sys usage is not clarified. Is it only limited to experts? Why only expert users were selected for the study? The collaborative nature of \sys seems to be suitable for non-experts also.}

\res{
	We apologize for the confusion. Indeed, \sys is designed to be used by both expert and non-expert users.
	
	To comprehensively evaluate \sys, we have invited additional five non-experts to participate in the user study. We have updated the user study results, demonstrating that \sys is also suitable for non-experts, as it not only recommends visualizations but also provides hints to guide further data exploration.
%
For detailed findings and analysis, please refer to \textbf{Exp-2} in \textbf{Sec}~\ref{sec:experiment}.
}


\subsection*{Responses to Reviewer \#5} 

\etitle{WEAK POINT W1:} \textit{Some details of the design choice need justification. D1, D2.}

\etitle{DETAIL D1:} \textit{While navigating the search space should be one bottleneck in improving the efficiency of VizRec systems and the experimental results show that the proposed method achieves good performance, more detailed analysis of MCGS compared to MCTS is expected. Sharing of information between nodes improves the efficiency, but is there a cost? Is it possible that one of two similar visualizations like Q1 and Q2 in Figure 6 will have high quality but get pruned when using MCGS? The authors need to provide more background/references or analysis of the search algorithm here.}

\res{Thank you for the insightful comments. 
	We have provided a detailed comparison of MCTS and MCGS at the end of \textbf{Sec}~\ref{sec:mcgs_vis_gen}, as suggested.
	Our analysis shows that MCGS, by using a graph structure instead of a tree structure, enables more effective sharing of information between nodes and reduces the number of nodes, thereby increasing search efficiency.
	
Moreover, our experiments demonstrate that \sys is, on average, 1.8 times faster than MCTS, especially for datasets with many columns. For example, when processing the VideoGame dataset with 15 columns, \sys's graph-based structure is 2.9 times faster than MCTS's tree-based structure. For more details, please refer to \textbf{Exp-7} in \textbf{Sec}~\ref{sec:experiment}.
	
 Regarding the pruning issue you mentioned, our rule-based pruning algorithm will only remove those low-quality visualizations that are syntactically incorrect or violate visualization rules. Therefore, all valid visualizations are reserved after the visualization generation stage, as detailed in \textbf{Sec}~\ref{sec:optim}.
}


\etitle{DETAIL D2-1:} \textit{The necessity of using a GAN is not clear.}

\res{Thank you for your comments. 
	Inspired by existing research~\cite{DBLP:journals/isci/GaoZYLWX21, zhu2020recommendation} for recommendation systems, we chose to use the GAN to learn user preferences offline. Specifically, we implemented the representative IRecGAN~\cite{DBLP:conf/nips/BaiGW19} method. While the GAN are not the only option, we have demonstrated good performance of the GAN model in our experiment (\textbf{Exp-5}).}


\etitle{DETAIL D2-2:} \textit{If each user has only 1.85 visualizations, is it really possible to learn the preferences? Why not clustering the users? }

\res{Sorry for the confusion. Actually, we employed the user clustering strategy, which is feasible with the real-world visualization corpus from the Plotly community~\cite{qian2022personalized}. This corpus includes concepts of visualization configurations, enabling us to learn preferences across datasets and users. By aggregating data features, user preferences, and visualization features across different datasets, we obtained 15,531 training samples to train the IRecGAN model. We have clarified this part in \textbf{Sec}~\ref{sec:learn_reward_function}, as suggested.}

% \res{}Sorry for the confusion. Actually, we considered a user clustering strategy, which is feasible with the PVisRec~\cite{qian2022personalized} dataset as it includes concepts of visualization configurations, allowing us to learn preferences across datasets and users. By aggregating data features, user features, and visualization features across different datasets, we obtained $15,531$ training samples to train the IRecGAN model. We have clarified this part in Section~\ref{sec:learn_reward_function}, as suggested.}

\etitle{DETAIL D2-3:} \textit{Is the GAN model trained on the fly when the real users are using the system (but even so, there are only a couple of rounds of interaction; I don't see how the personalized GAN is trained and evaluated)?}

\res{The GAN model is trained offline. The goal of the GAN model is to learn general user preferences from real-world visualization tasks. \sys utilizes the learning-to-rate component (with GAN as a part of this component) to generate a set of high-quality visualizations in the first round of visualization recommendations. During interactions, we capture changes in user preferences through visualization hints. Please refer to \textbf{Sec}~\ref{sec:learn_reward_function} for more details.}

\etitle{WEAK POINT W2:} \textit{Some evaluation settings need clarification. D3.}

\etitle{DETAIL D3:} \textit{What is the training data for all the methods? In section 5, it says that \sys uses 285,236 visualizations from~\cite{DBLP:conf/icde/LuoQ0018}, but in section 7, the VizML benchmark also provides training data. Is the proposed method trained on both datasets? Are baselines also trained on both? Clarifying the settings would be important to ensure the fairness of the experiments.}

\res{We apologize for the confusion. To clarify, we used the VizML corpus as the training data for all methods.
	
For a fair comparison, we trained our system using the VizML corpus, naming this version \sys-. As shown in Table~\ref{tab:init_rec_results}, \sys- trained on VizML still outperforms the state-of-the-art methods, demonstrating the effectiveness of our framework under the same evaluation settings. This ensures that all methods, including our proposed method and the baselines, are evaluated fairly and consistently.}


\etitle{WEAK POINT W3:} \textit{The problem definition in section 6 need clarification. D4, D5. }

\etitle{DETAIL D4:} \textit{Section 4 mentioned a number of iterations, and section 6 mentioned the budget of top-$k$ hints; they should be important parameters of the proposed solution and are the key to the trade-off between accuracy and efficiency. This paper will be strengthened with a sensitivity analysis of these parameters.}

\res{Thanks for the constructive comments.
%
We have conducted new experiments (\textbf{Exp-6} in \textbf{Sec}~\ref{sec:experiment}) to analyze the sensitivity of these parameters, as suggested. The results show that the number of iterations stabilizes performance within a specific range, such as 50 iterations, and beyond 100 iterations, the performance improvement is negligible. Therefore, setting a reasonable value like 100 iterations offers a better trade-off between accuracy and efficiency. Similarly, for the budget of top-$k$ hints, lower values like 10 provide limited hints and fail to meet user needs effectively. The results show that setting the budget to 40 or 50 offers stable performance, suggesting an appropriate parameter setting to ensure a trade-off between accuracy and efficiency. Please refer to \textbf{Exp-6} for details.}

% showing that \sys is stable and performs well with proper settings. Please refer to \textbf{Exp-6} in \textbf{Sec~\ref{sec:experiment}} for details.}


\etitle{DETAIL D5:} \textit{The problem definition in Sec 6 needs more justification. There is a pre-defined k for top-$k$ visualization hints, then why don't we have a pre-defined $l$ for top-$l$ visualization per hint? Is it feasible to show all visualizations for each hint (we don't even know how many visualizations are in total for one hint)? Even if the current definition may lead to higher reward values, I don't see why it is better than showing top-$l$ visualizations for top-$k$ hints.}

\res{Sorry for the confusion. The visualizations of each hint are ranked, and we show the ranked visualizations to users. 
We performed a sensitivity analysis on $l$ to evaluate its impact on recommendation performance. The results show that $l$ should be in a specific range for optimal results. A lower $l$ (\eg 1) fails to capture users' interests effectively, leading to poor performance. When $l$ is set to 8 or more, the hit rate stabilizes above 90\%, and further increasing $l$ offers no significant improvement. Therefore, the choice of $l$ should be within an appropriate range, as detailed in \textbf{Exp-6}.

We have revised the problem definition in Section~\ref{sec:recommendation}, as suggested.}

\etitle{WEAK POINT W4:} \textit{The user study can be better designed. D6}

\etitle{DETAIL D6:} \textit{A user study is great for showing the usefulness of the proposed solution. The user study could tell more --- if we replace \sys with any state-of-the-art visualization recommendation tool, I would imagine that users will still find it easy to learn, easy to use, and provides high-quality results. Therefore, the comparison with state-of-the-art visualization recommendation tools will be much more interesting, especially for the LLMs (e.g., GPT-4) that provide data analysis functionalities and allow the users to interact further.}


\res{Thanks for these good suggestions. We have improved our user study based on the comments.

First, we have extended our user study and invited five additional non-expert users.

Second, we have conducted a qualitative analysis of user comments and derived some new insights. For example, participants appreciated the intuitive hints provided by \sys, which guided them effectively through the data exploration process. However, some users mentioned the need for more customization options to tailor the visualizations to their specific needs.


Regarding the comparison with state-of-the-art visualization recommendation tools, we have performed a new comparison experiment with LLM4Vis~\cite{DBLP:conf/emnlp/WangZWLW23} in \textbf{Exp-1}. 
Additionally, we improved LLM4Vis by refining its prompt, allowing for data queries and top-$k$ visualization recommendations, denoted as LLM4Vis+.
We included LLM4Vis+ in our user study (\textbf{Exp-2}).

In summary, \sys is designed for exploratory data analysis and is suitable for scenarios where user intent is not well-defined. While tools such as NL2VIS may perform well in scenarios with clear user intent, our approach addresses different application needs. Please refer to the discussion on LLM4VIS in Section~\ref{sec:related} for details.
}

